FLAG n' FLARE: Fast Linearly-Coupled Adaptive Gradient Methods

We consider first order gradient methods for effectively optimizing a composite objective in the form of a sum of smooth and, potentially, non-smooth functions. We present accelerated and adaptive gradient methods, called FLAG and FLARE, which can offer the best of both worlds. They can achieve the optimal convergence rate by attaining the optimal first-order oracle complexity for smooth convex optimization. Additionally, they can adaptively and non-uniformly re-scale the gradient direction to adapt to the limited curvature available and conform to the geometry of the domain. We show theoretically and empirically that, through the compounding effects of acceleration and adaptivity, FLAG and FLARE can be highly effective for many data fitting and machine learning applications.

==> corrections.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[H]
\caption{WadaGrad}
\label{alg:wadagrad}
\begin{algorithmic}[1]
\INPUT $F=f+h$, $L$ lipschitz constant for $f$, constraint set $\C$, $\xx_1 = \yy_1 = \zz_1$, $T$
\For{k=1 to T}
\State $\yy_{k+1} \gets \prox(\xx_{k})$\;
\State \label{alg_step_grad_map} $\pp_k \gets -L(\yy_{k+1}-\xx_{k})$
\State $\vg_{k} \gets \pp_k /{\|\pp_k \|_2}$
\State \label{algstep:g_ik} $\vg_{1:k} \gets [\vg_{1:k-1}, \vg_{k}]$ \fred{Fix this notation for $\vg_{1:k}$ as it is a matrix}
\State \label{algstep:s_ki} $\vs_{k}(i) \gets \|\vg_{1:k,i}\|_2$ \fred{Change to familiar Matlab notation for slicing}
\State \label{algstep:S_k}$ S_k \gets \text{diag}(\vs_k) + \delta \mathbb{I}$
\State $\psi_k(\xx) \gets \frac{1}{2}\xx^T S_k \xx$
%\State $Prog_k \gets \frac{1}{2L}\|\pp_k \|_2^2$ 
%\State $Cost_k \gets \frac{1}{2}\|\pp_k \|_{\psi_k^*}^2$
\State \label{algstep:L_k} $L_k \gets L{ \pp_{k}^{T} S^{-1}_{k} \pp_{k}}/{\|\pp_{k}\|_{2}^{2}}$
\State $\eta_k \gets \text{ComputeMirrorStepsize}$
\State $\mu_k \gets \text{ComputeWeight}$
\State $\zz_{k+1} \gets \arg\min_{\zz\in \C} \lin{\eta_k \pp_k , \zz -\zz_{k}} + \hf \|\zz-\zz_{k}\|^{2}_{S_{k}}$
%\State $\zz_{k+1} \gets \arg\min_{\zz\in \C} \lin{\eta_k \pp_k , \zz -\zz_{k}} + B_{\psi_k}(\zz,\zz_{k})$
\State $\epsilon_{k} \gets {1}/\left(3 L T {\max \{\eta_{k} L_{k},1\} \| \yy_{k+1} - \zz_{k+1} \|_{2}^{2}}\right)$ 
\State $\xx_{k+1}\gets BinarySearch(\zz_{k+1},\yy_{k+1}, \epsilon_{k})$
\EndFor
\Return $\yy_{T+1}$
\end{algorithmic}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem} 
\label{t:mastertheorem}
Let $D \defeq \sup_{\xx, \yy \in \C} \|\xx - \yy\|_\infty^2$. For any $\uu \in \C$, after $T$ iterations of Algorithm \ref{alg:wadagrad}, we get
\begin{equation*}
\sum_{k=1}^T \eta_k (F(\yy_{k+1}) - F(\uu))   \leq 1 + \frac{D}{2}\|\vs_T\|_1 + \sum_{k=1}^T \textcolor{red}{(\eta_k^2L_k-\eta_k)}  \left( F(\yy_{k}) - F(\yy_{k+1}) \right).
\end{equation*}
%$$\sum_{k=1}^T \eta_k (F(\yy_{k}) - F(u)) \leq \sum_{k=1}^T (\eta_k^2 L_k - \eta_{k+1}^2 L_{k+1}) F(\yy_{k}) + 2D\|s_T\|_1$$
\end{theorem}

\begin{proof}
\begin{align}
&\quad \sum_{k=1}^T \eta_k(F(y_{k+1})-F(u))\\
\text{(by lemma \ref{lem:Ftf}) }
&\leq \sum_{k=1}^T \eta_k(\tf(y_{k+1})-\tf(u))\\
&= \sum_{k=1}^T \eta_k(\tf(x_{k})-\tf(u)) + \textcolor{red}{\eta_k(\tf(y_{k+1})-\tf(x_k))}\\
\text{(by convexity) }
&\leq \sum_{k=1}^T \eta_k\lin{\nabla \tf(x_k), (x_k - u)}\\
&= \sum_{k=1}^T \eta_k\lin{\tilde{\nabla}_k, (x_k - u)}\\
&= \sum_{k=1}^T \eta_k\lin{\tilde{\nabla}_k, (z_k - u)} + \sum_{k=1}^T\eta_k\lin{\tilde{\nabla}_k, x_k - z_k} \\
\label{line:122}
\text{(by corollary \ref{c:mir}) }&\leq 2D\|s_T\|_1 +\sum_{k=1}^T \frac{\eta_k^2}{2}\|\tilde{\nabla}_k\|^2_{\psi_k^*} + \sum_{k=1}^T\eta_k\lin{\tilde{\nabla}_k, x_k - z_k}\\
\label{l:central}
\text{(by lemma \ref{lem:proxavg}),letting $r=\eta_kL_k-1$) }
&\leq 2D\|s_T\|_1 +\sum_{k=1}^T \frac{\eta_k^2}{2}\|\tilde{\nabla}_k\|^2_{\psi_k^*} + \sum_{k=1}^T \textcolor{red}{(\eta_k^2 L_k-\eta_k)} \lin{\tilde{\nabla}_k, y_k - x_k}\\
\text{(by expression \ref{e:tildeftildek} and convexity of $\tilde{f}_k$) }
&\leq 2D\|s_T\|_1 +\sum_{k=1}^T \frac{\eta_k^2}{2}\|\tilde{\nabla}_k\|^2_{\psi_k^*} + \sum_{k=1}^T\textcolor{red}{(\eta_k^2 L_k-\eta_k)}(\tf(y_k) - \tf(x_k))\\
\text{(by definition of $L_k$ and lemma \ref{lem:tfprog}) }
&\leq 2D\|s_T\|_1 +\sum_{k=1}^T \eta_k^2 L_k (\tf(x_k) - \tf(y_{k+1}) + \sum_{k=1}^T\textcolor{red}{(\eta_k^2 L_k-\eta_k)}L_k (\tf(y_k) - \tf(x_k))\\
&=2D\|s_T\|_1 +\sum_{k=1}^T \textcolor{red}{(\eta_k^2 L_k-\eta_k)} (\tf(y_k) - \tf(y_{k+1}))\\
\text{(lemma \ref{lem:Ftf} with $u=y_{k}$) }
&\leq 2D\|s_T\|_1 +\sum_{k=1}^T \textcolor{red}{(\eta_k^2 L_k-\eta_k)} (F(y_k) - F(y_{k+1}))\\
\label{l:212}
\end{align}
$\qed$
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Correct Adaptive Stepsize}
We begin with the theorem
\begin{theorem}
\label{t:mastertheorem}
Let $D \defeq \sup_{\xx, \yy \in \C} \|\xx - \yy\|_\infty^2$. For any $\uu \in \C$, after $T$ iterations of Algorithm \ref{alg:wadagrad}, we get
\begin{equation*}
\sum_{k=1}^T \eta_k (F(\yy_{k+1}) - F(\uu))   \leq 1 + \frac{D}{2}\|\vs_T\|_1 + \sum_{k=1}^T(\eta_k^2 L_k - \eta_k) \left( F(\yy_{k}) - F(\yy_{k+1}) \right).
\end{equation*}
%$$\sum_{k=1}^T \eta_k (F(\yy_{k}) - F(u)) \leq \sum_{k=1}^T (\eta_k^2 L_k - \eta_{k+1}^2 L_{k+1}) F(\yy_{k}) + 2D\|s_T\|_1$$
\end{theorem}

\begin{lemma}
\label{lem:penpen}
$$\sum_{k=1}^T (\eta_k - (\eta_k^2 L_k - \eta_{k-1}^2 L_{k-1}))(F(\yy_k) - F(\uu)) + \eta_T^2L_T F(\yy_{T+1}) - \sum_{k=1}^T \eta_k F(\uu) \leq \frac{D}{2}\|s_T\|_1$$
\end{lemma}

\begin{proof}
This is simply re-indexing the summation in theorem \ref{t:mastertheorem} and simple algebra. Moving all the summations to the left side:

\begin{align*}
&\sum_{k=1}^T \eta_k (F(\yy_{k+1}) - F(\uu)) - \sum_{k=1}^T(\eta_k^2 L_k - \eta_k) \left( F(\yy_{k}) - F(\yy_{k+1}) \right)\\
= & \sum_{k=1}^T \eta_k (F(\yy_{k+1})) - \sum_{k=1}^T \eta_k (F(\uu)) - \sum_{k=1}^T(\eta_k^2 L_k - \eta_k) \left( F(\yy_{k})\right) + \sum_{k=1}^T(\eta_k^2 L_k - \eta_k) \left( F(\yy_{k+1}) \right)\\
= & \sum_{k=1}^{T+1} \eta_{k-1} (F(\yy_{k})) - \sum_{k=1}^T \eta_k (F(\uu)) - \sum_{k=1}^T(\eta_k^2 L_k - \eta_k) \left( F(\yy_{k})\right) + \sum_{k=1}^{T+1}(\eta_{k-1}^2 L_k - \eta_{k-1}) \left( F(\yy_{k}) \right)\\
= & \sum_{k-1}^{T} F(\yy_k) (\eta_{k-1} - \eta_k^2 L_k + \eta_k + \eta_{k-1}^2 L_{k-1} - \eta_{k-1}) + F(\yy_{T+1}) (\eta_{T} + \eta_{T}^2L_T - \eta_{T}) - \sum_{k=1}^{T} \eta_k F(u)\\
= & \sum_{k=1}^T (\eta_k - (\eta_k^2L_k - \eta_{k-1}^2 L_{k-1}))F(\yy_k)  + \eta_T^2L_T F(\yy_{T+1}) - \sum_{k=1}^T \eta_k F(u)
\end{align*}
\end{proof}

\begin{algorithm}[H]
\caption{ComputeMirrorStepsize}\label{alg:chooseeta}
\begin{algorithmic}[1]
\State $\frac{1}{c_k} \gets \frac{ \frac{k}{L_k} + \sqrt{(\frac{k}{L_k})^2 + 4k^2 (\frac{1}{L_k}) (\sum_{i-1}^{k-1} \frac{i}{c_i}) } }{2k^2}$
\State $\eta_k \gets \frac{k}{c_k}$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
\caption{ComputeWeight}\label{alg:choosemu}
\begin{algorithmic}[1]
\State $\mu_k \gets \eta_k - (\eta_k^2 L_k - \eta_{k-1}^2 L_{k-1})$
\end{algorithmic}
\end{algorithm}

\begin{lemma}
\label{lem:ck}
The choice of $c_k$ in \ref{alg:chooseeta} satisfies the equality
\begin{equation}
\label{e:ck}
\eta_k = \frac{k}{c_k} = \sqrt{\sum_{i=1}^k \frac{i}{c_i L_k}} 
\end{equation}
\end{lemma}
We begin with the equality in \ref{e:ck}:
\begin{align*}
\sqrt{\sum_{i=1}^k \frac{i}{c_i L_k}} &= \frac{k}{c_k}\\
\sum_{i=1}^k \frac{i}{c_i L_k} &= \frac{k^2}{c_k}\\
k^2 \frac{1}{c_k^2}  - (\frac{k}{L_k})\frac{1}{c_k} + \sum_{i=1}^{k-1} \frac{i}{c_i L_k}&=0
\end{align*}

The above is a quadratic polynomial in $\frac{1}{c_k}$, and one can verify that the definition of $\frac{1}{c_k}$ in Algorithm \ref{alg:chooseeta} is exactly the root-formula for this quadratic polynomial. The equality for $\eta_k$ is by definition.

\begin{corollary}
\label{cor:etak}
\begin{enumerate}
\item $\eta_k^2L_k = \sum_{i=1}^k \frac{i}{c_i}$
\item $\eta_k^2 L_k - \eta_{k-1}^2 L_{k-1} = \eta_k$
\item $\sum_{k=1}^T \eta_k  = \sum_{k=1}^T \frac{k}{c_k}= \eta_{T}^2L_T$
\item $\eta_k^2L_k - \eta_k \geq 0$
\end{enumerate}
\end{corollary}
\begin{proof}
\begin{enumerate}
\item Follows from lemma \ref{lem:ck}.
\item Follows from item 1.
\item Follows from item 1 and the definition of $\eta_k$.
\item Follows from item 1, the definition of $\eta_k$ and the positivity of $c_k$.
\end{enumerate}
\end{proof}

\begin{lemma}
\label{lem:pen}
$$F(\yy_{T+1}) = F(u) \leq \frac{D\|s_T\|_1}{\sum_{k=1}^T \frac{k}{c_k}}$$
\end{lemma}
\begin{proof}
Using item 2 in corollary \ref{cor:etak}, we see that $\eta_k - (\eta_k^2L_k-\eta_{k-1}^2L_{k-1})=0$. Substituting this equality into lemma \ref{lem:penpen}, the summation goes away and we are left with
$$\eta_T^2L_T F(\yy_{T+1}) - \sum_{k=1}^T \eta_k F(\uu) \leq \frac{D}{2}\|s_T\|_1$$
Finally, using item 3 of corollary \ref{cor:etak}, we get
$$\left(\sum_{k=1}^T \frac{k}{c_k}\right)(F(y_{T+1}-F(u)) \leq D\|s_T\|_1$$
Dividing the summation gives the lemma.
\end{proof}

Finally, it only remains to lower bound the magnitude of $\sum_{k=1}^T \frac{k}{c_k}$. We do this by induction.

\begin{lemma}
Let $Q = \sum_{k=1}^T L_k$. Then $$\sum_{k=1}^T \frac{k}{c_k}
\geq \frac{T^3}{10000Q}$$
\end{lemma}

\begin{proof}
Here, we present an alternate proof to lemma \ref{lem:simulation}. We begin with expression 

$$\sum_{k=1}^{T} \frac{k}{c_k} = \sum_{k=1}^{T-1}\frac{k}{c_k} +\frac{ \frac{T}{L_T} + \sqrt{(\frac{T}{L_T})^2 + 4T^2 (\frac{1}{L_T}) (\sum_{i-1}^{T-1} \frac{i}{c_i}) } }{2T^2}$$

Let's now assume by induction that if $\sum_{k=1}^{T-1} L_k = Q$, then $\sum_{k=1}^{T-1} \frac{k}{c_k} \geq \frac{(T-1)^3}{10000Q}$

We can easily verify the base case when $T=1$, since $c_1=\frac{1}{L_1} = \frac{1}{Q}$.

Now, let $Q = \sum_{k=1}^T L_k$ and let $\alpha = \frac{L_k}{Q}$. 
\begin{align*}
&\sum_{k=1}^T \frac{k}{c_k}\\
=& \sum_{k=1}^{T-1} \frac{k}{c_k} + \frac{T}{c_T}\\
\geq & \frac{(T-1)^3}{10000(1-\alpha)Q} + \frac{1}{2}\left( \frac{1}{L_T} + \sqrt{\frac{1}{L_T^2} + \frac{4}{\alpha Q} \frac{(T-1)^3}{10000(1-\alpha)Q}}\right)\\
\geq & \frac{(T-1)^3}{10000(1-\alpha)Q} + \frac{1}{2}\left( \sqrt{\frac{4}{\alpha Q}\frac{(T-1)^3}{10000(1-\alpha)Q}}\right)
\end{align*}

Where the last line follows from our inductive hypothesis and the definition of $c_T$.

Now we consider 2 cases:

Case 1: $(1-\alpha)\leq \frac{(T-1)^3}{T^3}$, in which case $\frac{(T-1)^3}{10000(1-\alpha)Q} \geq \frac{T^3}{10000Q}$ and we are done.

Case 2: $(1-\alpha)\geq \frac{(T-1)^3}{T^3}$, in which case $\alpha \leq \frac{T^3-(T-1)^3}{T^3}\leq \frac{7}{T}$. Thus
\begin{align*}
& \frac{(T-1)^3}{10000(1-\alpha)Q} + \frac{1}{2}\left( \sqrt{\frac{4}{\alpha Q}\frac{(T-1)^3}{10000(1-\alpha)Q}}\right)\\
\geq & \frac{(T-1)^3}{10000Q} + \frac{1}{2}\left( \sqrt{\frac{4 T}{7 Q}\frac{(T-1)^3}{10000Q}}\right)\\
\geq & \frac{(T-1)^3}{10000Q} + \frac{1}{2}\left( \sqrt{\frac{T^4}{140000Q^2}}\right)\\
\geq & \frac{(T-1)^3}{10000Q} + \frac{T^2}{760Q}\\
\geq & \frac{T^3}{10000Q}
\end{align*}

\begin{remark}
The ridiculously large constant of $10000$ is almost entirely an artefact of analysis. For example, by picking $\eta_k = \frac{k+10}{c_k}$, and going through the analysis more carefully, one can get a constant that is on the order of $~10$. In preliminary experiments, even with $\eta_k = \frac{k}{c_k}$, the factor is no more than $10$.
\end{remark}

\begin{theorem}
\label{thm:final}
$$F(y_{T+1}) - F(u) \leq \frac{10000q^2}{T}\frac{LD}{T^2}$$
Where $\frac{q^2}{T} = d\frac{\min_{\|s\|_1\leq d} \sum_{k=1}^T \vg_{k}^T S^{-1} \vg_{k}}{ \sum_{k=1}^T \vg_{k}^T I \vg_{k}}\in[1,d]$
\end{theorem}

\begin{proof}
The theorem follows immediately from substituting lemma \ref{lem:cklb} into lemma \ref{lem:gammak}. We then upper bound $Q$: $Q=\sum_{k=1}^T L_k = L\sum_{k=1}^T \|\vg_{k}\|_{\psi_k^*}^2\leq 2Lq$, where the inequality and the interval for $q$ follows from lemma \ref{lem:adareg}.
Finally, by definition of $s_k$, we have $\|\s_T|_1 = q$
$\qed$
\end{proof}
